Axion Dark Matter

Axions are well-motivated dark matter candidates with simple cosmological production mechanisms. They were originally introduced to solve the strong CP problem, but also arise in a wide range of extensions to the Standard Model. This Snowmass white paper summarizes axion phenomenology and outlines next-generation laboratory experiments proposed to detect axion dark matter. There are vibrant synergies with astrophysical searches and advances in instrumentation including quantum-enabled readout, high-Q resonators and cavities and large high-field magnets. This white paper outlines a clear roadmap to discovery, and shows that the US is well-positioned to be at the forefront of the search for axion dark matter in the coming decade.

==> Snowmass2021_AxionPaper_AuthorList_2022_11_15_revtex.tex <==
\author{C.~B.~Adams}
\affiliation{Columbia University, New York, NY, USA}

\author{N.~Aggarwal}
\affiliation{Northwestern University, Evanston, IL, USA}

\author{A.~Agrawal}
\affiliation{University of Chicago, Chicago, IL, USA}

\author{R.~Balafendiev}
%\affiliation{School of Physics and Engineering, ITMO University, St. Petersburg, Russia}

\author{C.~Bartram}
\affiliation{University of Washington, Seattle, WA, USA}

\author{M.~Baryakhtar}
\affiliation{University of Washington, Seattle, WA, USA}

\author{H.~Bekker}
\affiliation{Helmholtz Institute (GSI) Mainz, Mainz, Germany}
\affiliation{Johannes Gutenberg University, Mainz, Mainz, Germany}

\author{P.~Belov}
%\affiliation{School of Physics and Engineering, ITMO University, St. Petersburg, Russia}

\author{K.~K.~Berggren}
\affiliation{Department of Electrical Engineering, Massachusetts Institute of Technology, Cambridge, MA, USA}

\author{A.~Berlin}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{C.~Boutan}
\affiliation{Pacific Northwest National Laboratory, Richland, WA, USA}

\author{D.~Bowring}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{D.~Budker}
\affiliation{Helmholtz Institute (GSI) Mainz, Mainz, Germany}
\affiliation{Johannes Gutenberg University, Mainz, Mainz, Germany}
\affiliation{University of California, Berkeley, Berkeley, CA, USA}

\author{A.~Caldwell}
\affiliation{Max-Planck-Institut f\"ur Physik, Munich, Germany}

\author{P.~Carenza}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, Stockholm, Sweden}

\author{G.~Carosi}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA , USA}
\affiliation{University of Washington, Seattle, WA, USA}

\author{R.~Cervantes}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{S.~S.~Chakrabarty}
\affiliation{Istituto Nazionale Fisica Nucleare, Sezione di Torino, Torino, Italy}

\author{S.~Chaudhuri}
\affiliation{Princeton University Department of Physics, Princeton, NJ, USA}

\author{T.~Y.~Chen}
\affiliation{Columbia University, New York, NY, USA}

\author{S.~Cheong}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}

\author{A.~Chou}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{R.~T.~Co}
\affiliation{William I. Fine Theoretical Physics Institute, School of Physics and Astronomy, University of Minnesota, Minneapolis, MN, USA}

\author{J.~Conrad}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, Stockholm, Sweden}

\author{D.~Croon}
\affiliation{Institute for Particle Physics Phenomenology, Durham University, Durham DH1 3LE, UK}

\author{R.~T.~D'Agnolo}
\affiliation{Universit\'e Paris-Saclay, CEA, Institut de Physique Th\'eorique, Gif-sur-Yvette, France}

\author{M.~Demarteau}
\affiliation{Oak Ridge National Laboratory, Oak Ridge, TN, USA}

\author{N.~DePorzio}
\affiliation{Department of Physics, Harvard University, Cambridge, MA, USA}

%\author{A.~V.~Derbin}
%\affiliation{Petersburg Nuclear Physics Institute NRC Kurchatov Institute, St. Petersburg, Russia}

\author{M.~Descalle}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA , USA}

\author{K.~Desch}
\affiliation{University of Bonn, Bonn, Germany}

\author{L.~Di~Luzio}
\affiliation{Dipartimento di Fisica e Astronomia 'G. Galilei', Universit\`a di Padova, Padova, Italy}
\affiliation{Istituto Nazionale Fisica Nucleare, Sezione di Padova, Padova, Italy}

\author{A.~Diaz-Morcillo}
\affiliation{Department of Information and Communications Technologies, Technical University of Cartagena, Cartagena, Spain}

\author{K.~Dona}
\affiliation{University of Chicago, Chicago, IL, USA}

%\author{I.~S.~Drachnev}
%\affiliation{Petersburg Nuclear Physics Institute NRC Kurchatov Institute, St. Petersburg, Russia}

\author{A.~Droster}
\affiliation{University of California, Berkeley, Berkeley, CA, USA}

\author{N.~Du}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA , USA}

\author{K.~Dunne}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, Stockholm, Sweden}

\author{B.~D\"obrich}
\affiliation{European Organization for Nuclear Research, Geneva, Switzerland}
\affiliation{Max-Planck-Institut f\"ur Physik, Munich, Germany}

\author{S.~A.~R.~Ellis}
\affiliation{D\'epartement de Physique Th\'eorique, Universit\'e de Gen\`eve, Gen\`eve, Switzerland}

\author{R.~Essig}
\affiliation{C.N. Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, NY, USA}

\author{J.~Fan}
\affiliation{Physics Department, Brown University, Providence, RI, USA}

\author{J.~W.~Foster}
\affiliation{Center for Theoretical Physics, Massachusetts Institute of Technology, Cambridge, MA, USA}

\author{J.~T.~Fry}
\affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA, USA}

\author{A.~Gallo~Rosso}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, Stockholm, Sweden}

\author{J.~M.~Garc{\'\i}a~Barcel\'o}
\affiliation{Department of Information and Communications Technologies, Technical University of Cartagena, Cartagena, Spain}

\author{I.~G.~Irastorza}
\affiliation{Centro de Astropart{\'\i}culas y F{\'\i}sica de Altas Energ{\'\i}as, Universidad de Zaragoza, Zaragoza, Spain}

\author{S.~Gardner}
\affiliation{University of Kentucky, Lexington, KY, USA}

\author{A.~A.~Geraci}
\affiliation{Northwestern University, Evanston, IL, USA}

\author{S.~Ghosh}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\affiliation{Department of Applied Physics, Yale University, New Haven, Connecticut, USA}

\author{B.~Giaccone}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{M.~Giannotti}
\affiliation{Barry University, Miami Shores, FL, USA}

\author{B.~Gimeno}
\affiliation{Instituto de F{\'\i}sica Corpuscular (CSIC - University of Valencia), Paterna (Valencia), Spain}

\author{D.~Grin}
\affiliation{Haverford College, Haverford, PA, USA}

\author{H.~Grote}
\affiliation{Gravity Exploration Institute, Cardiff University, Cardiff, United Kingdom}

\author{M.~Guzzetti}
\affiliation{University of Washington, Seattle, WA, USA}

\author{M.~H.~Awida}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{R.~Henning}
\affiliation{Department of Physics and Astronomy, University of North Carolina, Chapel Hill, Chapel Hill, North Carolina, USA}
\affiliation{Triangle Universities Nuclear Laboratory, Durham, NC, USA}

\author{S.~Hoof}
\affiliation{Institut f\"ur Astrophysik und Geophysik, Georg-August-Universit\"at G\"ottingen, G\"ottingen, Germany}

\author{G.~Hoshino}
\affiliation{University of Chicago, Chicago, IL, USA}

\author{V.~Irsic}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Cambridge, United Kingdom}
\affiliation{Cavendish Laboratory, University Cambridge, Cambridge, United Kingdom}

\author{K.~D.~Irwin}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}

\author{H.~Jackson}
\affiliation{University of California, Berkeley, Berkeley, CA, USA}

\author{D.~F.~Jackson~Kimball}
\affiliation{Department of Physics, Californina State University - East Bay, Hayward, California, USA}

\author{J.~Jaeckel}
\affiliation{Institut fuer theoretische Physik, Universitaet Heidelberg, Heidelberg, Germany}

\author{K.~Jakovcic}
\affiliation{Rudjer Boskovic Institute, Zagreb, Croatia}

\author{M.~J.~Jewell}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}

\author{M.~Kagan}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}

\author{Y.~Kahn}
\affiliation{Department of Physics, University of Illinois at Urbana-Champaign, Urbana, IL, USA}

\author{R.~Khatiwada}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}
\affiliation{Illinois Institute of Technology, Chicago, IL, USA}

\author{S.~Knirck}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{T.~Kovachy}
\affiliation{Northwestern University, Evanston, IL, USA}

\author{P.~Krueger}
\affiliation{Physikalisch-Technische Bundesanstalt, Braunschweig, Germany}

\author{S.~E.~Kuenstner}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}

\author{N.~A.~Kurinsky}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}
\affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA, USA}

\author{R.~K.~Leane}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}
\affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA, USA}

\author{A.~F.~Leder}
\affiliation{University of California, Berkeley, Berkeley, CA, USA}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA, USA}

\author{C.~Lee}
\affiliation{Max-Planck-Institut f\"ur Physik, Munich, Germany}

\author{K.~W.~Lehnert}
\affiliation{JILA, National Institute of Standards and Technology and University of Colorado, Boulder, CO, USA}
\affiliation{National Institute of Standards and Technology, Boulder, CO, USA}
\affiliation{Department of Physics, University of Colorado, Boulder, CO, USA}

\author{E.~W.~Lentz}
\affiliation{Pacific Northwest National Laboratory, Richland, WA, USA}

\author{S.~M.~Lewis}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{J.~Liu}
\affiliation{Cavendish Laboratory, University Cambridge, Cambridge, United Kingdom}

\author{M.~Lynn}
\affiliation{University of Chicago, Chicago, IL, USA}

\author{B.~Majorovits}
\affiliation{Max-Planck-Institut f\"ur Physik, Munich, Germany}

\author{D.~J.~E.~Marsh}
\affiliation{Theoretical Particle Physics and Cosmology, King's College London, London, United Kingdom}

\author{R.~H.~Maruyama}
\affiliation{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}

\author{B.~T.~McAllister}
\affiliation{ARC Centre of Excellence for Dark Matter Particle Physics, Deptartment of Physics, The University of Western Australia, Crawley, WA, Australia}
\affiliation{ARC Centre of Excellence for Dark Matter Particle Physics, Swinburne University of Technology, John St, Hawthorn VIC 3122, Australia}

\author{A.~J.~Millar}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, Stockholm, Sweden}
\affiliation{Nordita, KTH Royal Institute of Technology and Stockholm University, Stockholm, Sweden}

\author{D.~W.~Miller}
\affiliation{University of Chicago, Chicago, IL, USA}

\author{J.~Mitchell}
\affiliation{Cavendish Laboratory, University Cambridge, Cambridge, United Kingdom}

\author{S.~Morampudi}
\affiliation{Center for Theoretical Physics, Massachusetts Institute of Technology, Cambridge, MA, USA}

\author{G.~Mueller}
\affiliation{University of Florida, Gainesville, FL, USA}

%\author{V.~N.~Muratova}
%\affiliation{Petersburg Nuclear Physics Institute NRC Kurchatov Institute, St. Petersburg, Russia}

\author{S.~Nagaitsev}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}
\affiliation{University of Chicago, Chicago, IL, USA}

\author{E.~Nardi}
\affiliation{Istituto Nazionale Fisica Nucleare, Laboratori Nazionali di Frascati, Frascati, Italy}

\author{O.~Noroozian}
\affiliation{The National Aeronautics and Space Administration (NASA), Washington, D.C., USA}

\author{C.~A.~J.~O'Hare}
\affiliation{School of Physics, The University of Sydney, Camperdown, NSW, Australia}

\author{N.~S.~Oblath}
\affiliation{Pacific Northwest National Laboratory, Richland, WA, USA}

\author{J.~L.~Ouellet}
\affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA, USA}

\author{K.~M.~W.~Pappas}
\affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA, USA}

\author{H.~V.~Peiris}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, Stockholm, Sweden}

\author{K.~Perez}
\affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA, USA}
\affiliation{Columbia University, New York, NY, USA}

\author{A.~Phipps}
\affiliation{Department of Physics, Californina State University - East Bay, Hayward, California, USA}

\author{M.~J.~Pivovaroff}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA , USA}

\author{N.~M.~Rapidis}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}

\author{V.~H.~Robles}
\affiliation{Yale Center for Astronomy and Astrophysics, Department of Physics, Yale University, New Haven, Connecticut, USA}

\author{K.~K.~Rogers}
\affiliation{Dunlap Institute for Astronomy \& Astrophysics, University of Toronto, Toronto, ON, Canada}

\author{J.~Rudolph}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}

\author{J.~Ruz}
\affiliation{Centro de Astropart{\'\i}culas y F{\'\i}sica de Altas Energ{\'\i}as, Universidad de Zaragoza, Zaragoza, Spain}

\author{G.~Rybka}
\affiliation{University of Washington, Seattle, WA, USA}

\author{M.~Safdari}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}

\author{B.~R.~Safdi}
\affiliation{University of California, Berkeley, Berkeley, CA, USA}

\author{M.~S.~Safronova}
\affiliation{Department of Physics and Astronomy, University of Delaware, Newark, DE, USA}

\author{C.~P.~Salemi}
\affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA, USA}

\author{P.~Schuster}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}

\author{A.~Schwartzman}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}

\author{J.~Shu}
\affiliation{CAS Key Laboratory of Theoretical Physics, Institute of Thereotical Physics, Chinese Academy of Science, Beijing, P.R.China}

\author{M.~Simanovskaia}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}

\author{J.~Singh}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}

\author{S.~Singh}
\affiliation{Department of Electrical and Computer Engineering, University of Delaware, Newark, DE, USA}
\affiliation{Department of Physics and Astronomy, University of Delaware, Newark, DE, USA}

\author{K.~Sinha}
\affiliation{Department of  Physics and Astronomy, University of Oklahoma, Norman, OK, USA}

\author{J.~T.~Sinnis}
\affiliation{University of Washington, Seattle, WA, USA}

\author{M.~Siodlaczek}
\affiliation{European Organization for Nuclear Research, Geneva, Switzerland}

\author{M.~S.~Smith}
\affiliation{Oak Ridge National Laboratory, Oak Ridge, TN, USA}

\author{W.~M.~Snow}
\affiliation{Indiana University Center for Spacetime Symmetries, Bloomington, IN, USA}

\author{A.~Sonnenschein}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{D.~H.~Speller}
\affiliation{Johns Hopkins University, Baltimore, MD, USA}

\author{Y.~V.~Stadnik}
\affiliation{School of Physics, The University of Sydney, Camperdown, NSW, Australia}

\author{C.~Sun}
\affiliation{School of Physics and Astronomy, Tel-Aviv University, Tel-Aviv, Israel}

\author{A.~O.~Sushkov}
\affiliation{Boston Universitry, Boston, MA, USA}

\author{T.~M.~P.~Tait}
\affiliation{University of California, Irvine, Irvine, CA, USA}

\author{V.~Takhistov}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), UTIAS, The University of Tokyo, Kashiwa, Japan}

\author{D.~B.~Tanner}
\affiliation{University of Florida, Gainesville, FL, USA}

\author{F.~Tavecchio}
\affiliation{INAF-Osservatorio Astronomico di Brera, Merate, Italy}

\author{D.~J.~Temples}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{J.~H.~Thomas}
\affiliation{Illinois Institute of Technology, Chicago, IL, USA}

\author{M.~E.~Tobar}
\affiliation{ARC Centre of Excellence for Dark Matter Particle Physics, Deptartment of Physics, The University of Western Australia, Crawley, WA, Australia}

\author{N.~Toro}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}

\author{Y.~-D.~Tsai}
\affiliation{University of California, Irvine, Irvine, CA, USA}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL, USA}

\author{E.~C.~van~Assendelft~}
\affiliation{Physics Department, Stanford University, Stanford, CA, USA}

\author{K.~van~Bibber}
\affiliation{University of California, Berkeley, Berkeley, CA, USA}

\author{M.~Vandegar}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}

\author{L.~Visinelli}
\affiliation{Tsung-Dao Lee Institute, Shanghai, P.R. China}
\affiliation{School of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai, P.R. China}

\author{E.~Vitagliano}
\affiliation{University of California, Los Angeles, Los Angeles, CA, USA}

\author{J.~K.~Vogel}
\affiliation{Centro de Astropart{\'\i}culas y F{\'\i}sica de Altas Energ{\'\i}as, Universidad de Zaragoza, Zaragoza, Spain}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA , USA}

\author{Z.~Wang}
\affiliation{Center for Cosmology and Particle Physics, Department of Physics, New York University, New York, NY, USA}

\author{A.~Wickenbrock}
\affiliation{Johannes Gutenberg University, Mainz, Mainz, Germany}
\affiliation{Helmholtz Institute (GSI) Mainz, Mainz, Germany}

\author{L.~Winslow}
\affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA, USA}

\author{S.~Withington}
\affiliation{Cavendish Laboratory, University Cambridge, Cambridge, United Kingdom}

\author{M.~Wooten}
\affiliation{University of California, Berkeley, Berkeley, CA, USA}

\author{J.~Yang}
\affiliation{Pacific Northwest National Laboratory, Richland, WA, USA}

\author{B.~A.~Young}
\affiliation{Santa Clara University, Santa Clara, CA, USA}

\author{F.~Yu}
\affiliation{PRISMA$^+$ Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, Mainz, Germany}

\author{K.~Zhou}
\affiliation{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}

\author{T.~Zhou}
\affiliation{Department of Electrical Engineering, Massachusetts Institute of Technology, Cambridge, MA, USA}


==> author_list_old.tex <==

\author[1]{Gray Rybka}
\author[2]{Maurizio Giannotti}
\author[3]{Derek F. Jackson Kimball}
\author[4]{Chen~Sun}
\author[5]{Edoardo Vitagliano}
\author[6]{Yevgeny V.~Stadnik}
\author[7]{Yu-Dai~Tsai}
\author[8,9]{Alexander~J.~Millar}
\author[10]{Sebastian Hoof}
\author[11]{Chang Lee}
\author[12]{Andrew Sonnenschein}
\author[12]{Stefan Knirck}
\author[13]{Jesse Liu}
\author[14]{Erik W.~Lentz}
\author[14]{Noah S. Oblath}
\author[15]{Nicholas DePorzio}
\author[16]{Michael E. Tobar}
\author[16]{Benjamin T. McAllister}
\author[17]{Andrew A. Geraci}
\author[18]{Kevin Zhou}
\author[19]{Volodymyr Takhistov}
\author[20]{Raymond T. Co}
\author[21,22]{Arne Wickenbrock}
\author[21,22]{Hendrik Bekker}
\author[23]{Colin Adams}
\author[24]{Zihui Wang}
\author[25]{Asher Berlin}
\author[26]{Sebastian~A.~R.~Ellis}
\author[27]{Raffaele~Tito~D'Agnolo}
\author[28]{Anton Sokolov}
\author[29]{Pablo Quilez}
\author[6,30]{Ciaran~A.~J.~O'Hare}
\author[31]{Joerg Jaeckel}
\author[32]{Babette D\"obrich}
\author[33]{J.M. García Barceló}
\author[12]{Mohamed H. Awida}
\author[34]{Victor H. Robles}
\author[35]{David W. Miller}
\author[36]{Joshua W. Foster}
\author[37,38,39]{Christopher Dessert}

 
\affil[1]{University of Washington}
\affil[2]{Department of Chemistry and Physics, Barry University, 11300 NE 2nd Ave., Miami Shores, FL 33161, USA}
\affil[3]{Department of Physics, California State University -- East Bay, Hayward, California 94542, USA}
\affil[4]{School of Physics and Astronomy, Tel-Aviv University, Tel-Aviv 69978, Israel}
\affil[5]{Department of Physics and Astronomy, University of California, Los Angeles, California 90095-1547, USA}
\affil[6]{School of Physics, The University of Sydney, NSW 2006, Australia}
\affil[7]{University of California, Irvine}
\affil[8]{The Oskar Klein Centre for Cosmoparticle Physics,
Department of Physics, Stockholm University}
\affil[9]{Nordita, KTH Royal Institute of Technology and Stockholm University}
\affil[10]{Institut f\"ur Astrophysik und Geophysik, Georg-August-Universtit\"at G\"ottingen, Friedrich-Hund-Platz~1, 37077 G\"ottingen, Germany}
\affil[11]{Max Planck Institute for Physics, 80805 Munich, Germany}
\affil[12]{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\affil[13]{Cavendish Laboratory, University of Cambridge, Cambridge CB3 0HE, UK}
\affil[14]{Pacific Northwest National Laboratory, Richland, WA 99354 USA}
\affil[15]{Department of Physics, Harvard University, Cambridge, MA 02138, USA}
\affil[16]{ARC Centre of Excellence for Dark Matter Particle Physics, Department of Physics, The University of Western Australia, WA, 6009, Australia}
\affil[17]{Center for Fundamental Physics, Department of Physics and Astronomy, Northwestern University, Evanston, IL 60208, USA}
\affil[18]{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, Menlo Park, CA 94025, USA}
\affil[19]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), UTIAS \\The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\affil[20]{William I. Fine Theoretical Physics Institute, School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\affil[21]{Johannes Gutenberg-Universit{\"a}t Mainz, 55128 Mainz, Germany}
\affil[22]{Helmholtz-Institut Mainz, GSI Helmholtzzentrum f{\"u}r Schwerionenforschung, 55128 Mainz, Germany} 
\affil[23]{Physics Department, Columbia University, New York, NY 10027, USA}
\affil[24]{Center for Cosmology and Particle Physics, Department of Physics, New York University, New York, NY 10003, USA}
\affil[25]{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\affil[26]{D\'epartement de Physique Th\'eorique, Universit\'e de Gen\`eve,\\
24 quai Ernest Ansermet, 1211 Gen\`eve 4, Switzerland}
\affil[27]{Universit\'e Paris Saclay, CEA, CNRS, Institut de Physique Th\'eorique, 91191, Gif-sur-Yvette, France}
\affil[28]{Deutsches Elektronen-Synchrotron DESY, Notkestra\ss e 85, D-22607 Hamburg, Germany}
\affil[29]{Deutsches Elektronen-Synchrotron DESY, Notkestra\ss e 85, D-22607 Hamburg, Germany}
\affil[30]{ARC Centre of Excellence for Dark Matter Particle Physics, Sydney, Australia}
\affil[31]{Institute for Theoretical Physics, Heidelberg University, Philosophenweg 16, 69120 Heidelberg Germany}
\affil[32]{CERN, Esplanade des Particules 1, 1211 Geneva, Switzerland}
\affil[33]{Department of Information and Communications Technologies, Technical University of Cartagena, 30203 - Cartagena, Spain}
\affil[34]{Physics Department, Yale Center for Astronomy and Astrophysics, New Haven, CT 06520, USA}
\affil[35]{Enrico Fermi Institute and The University of Chicago, Chicago, IL 60637, USA}
\affil[36]{Center for Theoretical Physics, Massachusetts Institute of Technology, Cambridge, Massachusetts 02139, U.S.A}
\affil[37]{Leinweber Center for Theoretical Physics, Department of Physics, University of Michigan, Ann Arbor, MI 48109 U.S.A.}
\affil[38]{Berkeley Center for Theoretical Physics, University of California, Berkeley, CA 94720, U.S.A.}
\affil[39]{Theoretical Physics Group, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, U.S.A.}
%How to associate two affiliations? 24,25 are both for Arne Wickenbrock
% Long author lists can be formatted and imported
% Feel free to list additional authors/endorser at the end of the document
%\input{authors.tex}


==> axions_author_list.tex <==
\author[1]{C.~B.~Adams}
\author[2]{A.~Agrawal}
\author[3]{R.~Balafendiev}
\author[4]{C.~Bartram}
\author[4]{M.~Baryakhtar}
\author[5,6]{H.~Bekker}
\author[3]{P.~Belov}
\author[7]{K.~K.~Berggren}
\author[8]{A.~Berlin}
\author[9]{C.~Boutan}
\author[8]{D.~Bowring}
\author[5,6,10]{D.~Budker}
\author[11,4]{G.~Carosi}
\author[12]{S.~S.~Chakrabarty}
\author[13]{S.~Chaudhuri}
\author[14,15]{S.~Cheong}
\author[8]{A.~Chou}
\author[16]{R.~T.~Co}
\author[17]{J.~Conrad}
\author[18]{R.~T.~D'Agnolo}
\author[19]{M.~Demarteau}
\author[20]{N.~DePorzio}
\author[21]{A.~V.~Derbin}
\author[22,23]{L.~Di~Luzio}
\author[24]{A.~Diaz-Morcillo}
\author[10]{A.~Droster}
\author[11]{N.~Du}
\author[17]{K.~Dunne}
\author[25]{B.~D\"obrich}
\author[26]{S.~A.~R.~Ellis}
\author[27]{R.~Essig}
\author[28]{J.~Fan}
\author[29]{J.~W.~Foster}
\author[30]{J.~T.~Fry}
\author[17]{A.~Gallo~Rosso}
\author[24]{J.~M.~Garc{\'\i}a~Barcel\'o}
\author[31]{I.~G.~Irastorza}
\author[32]{S.~Gardner}
\author[33]{A.~A.~Geraci}
\author[34,35]{S.~Ghosh}
\author[36]{M.~Giannotti}
\author[37]{B.~Gimeno}
\author[38]{D.~Grin}
\author[39]{H.~Grote}
\author[4]{M.~Guzzetti}
\author[8]{M.~H.~Awida}
\author[40,41]{R.~Henning}
\author[42]{S.~Hoof}
\author[43,44]{V.~Irsic}
\author[10]{H.~Jackson}
\author[45]{D.~F.~Jackson~Kimball}
\author[46]{J.~Jaeckel}
\author[14]{M.~Kagan}
\author[47]{Y.~Kahn}
\author[8,48]{R.~Khatiwada}
\author[8]{S.~Knirck}
\author[33]{T.~Kovachy}
\author[49]{P.~Krueger}
\author[15]{S.~E.~Kuenstner}
\author[14,50]{N.~A.~Kurinsky}
\author[14,50]{R.~K.~Leane}
\author[10,51]{A.~F.~Leder}
\author[52]{C.~Lee}
\author[53,54,55]{K.~W.~Lehnert}
\author[9]{E.~Lentz}
\author[8]{S.~M.~Lewis}
\author[56]{A.~Lindner}
\author[44]{J.~Liu}
\author[2]{M.~Lynn}
\author[57]{B.~Majorovits}
\author[58]{D.~J.~E.~Marsh}
\author[34]{R.~H.~Maruyama}
\author[59,60]{B.~T.~McAllister}
\author[17,61]{A.~J.~Millar}
\author[2]{D.~W.~Miller}
\author[29]{S.~Morampudi}
\author[62]{G.~Mueller}
\author[21]{V.~N.~Muratova}
\author[8,2]{S.~Nagaitsev}
\author[63]{O.~Noroozian}
\author[64]{C.~A.~J.~O'Hare}
\author[9]{N.~S.~Oblath}
\author[30]{J.~L.~Ouellet}
\author[30]{K.~M.~W.~Pappas}
\author[17]{H.~V.~Peiris}
\author[30]{K.~Perez}
\author[45]{A.~Phipps}
\author[11]{M.~J.~Pivovaroff}
\author[56]{P.~Qu\'ilez}
\author[15]{N.~M.~Rapidis}
\author[65]{V.~H.~Robles}
\author[66]{K.~K.~Rogers}
\author[15]{J.~Rudolph}
\author[31]{J.~Ruz}
\author[4]{G.~Rybka}
\author[14,15]{M.~Safdari}
\author[10]{B.~R.~Safdi}
\author[67]{M.~S.~Safronova}
\author[30]{C.~P.~Salemi}
\author[56]{J.~Schaffran}
\author[14]{P.~Schuster}
\author[14]{A.~Schwartzman}
\author[68]{J.~Shu}
\author[15]{M.~Simanovskaia}
\author[15]{J.~Singh}
\author[69,67]{S.~Singh}
\author[70]{K.~Sinha}
\author[4]{J.~T.~Sinnis}
\author[25]{M.~Siodlaczek}
\author[19]{M.~S.~Smith}
\author[71]{W.~M.~Snow}
\author[56]{A.~Sokolov}
\author[8]{A.~Sonnenschein}
\author[72]{D.~H.~Speller}
\author[64]{Y.~V.~Stadnik}
\author[82]{C.~Sun}
\author[73]{A.~O.~Sushkov}
\author[74]{T.~M.~P.~Tait}
\author[75]{V.~Takhistov}
\author[62]{D.~B.~Tanner}
\author[8]{D.~J.~Temples}
\author[48]{J.~H.~Thomas}
\author[59]{M.~E.~Tobar}
\author[14]{N.~Toro}
\author[74,8]{Y.-D.~Tsai}
\author[10]{K.~van~Bibber}
\author[14]{M.~Vandegar}
\author[76,77]{L.~Visinelli}
\author[78]{E.~Vitagliano}
\author[31,11]{J.~K.~Vogel}
\author[79]{Z.~Wang}
\author[6,5]{A.~Wickenbrock}
\author[30]{L.~Winslow}
\author[44]{S.~Withington}
\author[10]{M.~Wooten}
\author[9]{J.~Yang}
\author[80]{B.~A.~Young}
\author[81]{F.~Yu}
\author[14]{K.~Zhou}
\author[7]{T.~Zhou}

\affil[1]{Columbia University, New York, NY, USA}
\affil[2]{University of Chicago, Chicago, IL, USA}
\affil[3]{School of Physics and Engineering, ITMO University, St. Petersburg, Russia}
\affil[4]{University of Washington, Seattle, WA, USA}
\affil[5]{Helmholtz Institute (GSI) Mainz, Mainz, Germany}
\affil[6]{Johannes Gutenberg University, Mainz, Mainz, Germany}
\affil[7]{Department of Electrical Engineering, Massachusetts Institute of Technology, Cambridge, MA, USA}
\affil[8]{Fermi National Accelerator Laboratory, Batavia, IL, USA}
\affil[9]{Pacific Northwest National Laboratory, Richland, WA, USA}
\affil[10]{University of California, Berkeley, Berkeley, CA, USA}
\affil[11]{Lawrence Livermore National Laboratory, Livermore, CA , USA}
\affil[12]{Istituto Nazionale Fisica Nucleare, Sezione di Torino, Torino, Italy}
\affil[13]{Princeton University Department of Physics, Princeton, NJ, USA}
\affil[14]{Fundamental Physics Directorate, SLAC National Accelerator Laboratory, Menlo Park, CA, USA}
\affil[15]{Physics Department, Stanford University, Stanford, CA, USA}
\affil[16]{William I. Fine Theoretical Physics Institute, School of Physics and Astronomy, University of Minnesota, Minneapolis, MN, USA}
\affil[17]{The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, Stockholm, Sweden}
\affil[18]{Universit\'e Paris-Saclay, CEA, Institut de Physique Th\'eorique, Gif-sur-Yvette, France}
\affil[19]{Oak Ridge National Laboratory, Oak Ridge, TN, USA}
\affil[20]{Department of Physics, Harvard University, Cambridge, MA, USA}
\affil[21]{Petersburg Nuclear Physics Institute NRC Kurchatov Institute, St. Petersburg, Russia}
\affil[22]{Dipartimento di Fisica e Astronomia 'G. Galilei', Universit\`a di Padova, Padova, Italy}
\affil[23]{Istituto Nazionale Fisica Nucleare, Sezione di Padova, Padova, Italy}
\affil[24]{Department of Information and Communications Technologies, Technical University of Cartagena, Cartagena, Spain}
\affil[25]{European Organization for Nuclear Research, Geneva, Switzerland}
\affil[26]{D\'epartement de Physique Th\'eorique, Universit\'e de Gen\`eve, Gen\`eve, Switzerland}
\affil[27]{C.N. Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, NY, USA}
\affil[28]{Physics Department, Brown University, Providence, RI, USA}
\affil[29]{Center for Theoretical Physics, Massachusetts Institute of Technology, Cambridge, MA, USA}
\affil[30]{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA, USA}
\affil[31]{Centro de Astropart{\'\i}culas y F{\'\i}sica de Altas Energ{\'\i}as, Universidad de Zaragoza, Zaragoza, Spain}
\affil[32]{University of Kentucky, Lexington, KY, USA}
\affil[33]{Northwestern University, Evanston, IL, USA}
\affil[34]{Wright Laboratory, Department of Physics, Yale University, New Haven, Connecticut, USA}
\affil[35]{Department of Applied Physics, Yale University, New Haven, Connecticut, USA}
\affil[36]{Barry University, Miami Shores, FL, USA}
\affil[37]{Instituto de F{\'\i}sica Corpuscular (CSIC - University of Valencia), Paterna (Valencia), Spain}
\affil[38]{Haverford College, Haverford, PA, USA}
\affil[39]{Gravity Exploration Institute, Cardiff University, Cardiff, United Kingdom}
\affil[40]{Department of Physics and Astronomy, University of North Carolina, Chapel Hill, Chapel Hill, North Carolina, USA}
\affil[41]{Triangle Universities Nuclear Laboratory, Durham, NC, USA}
\affil[42]{Institut f\"ur Astrophysik und Geophysik, Georg-August-Universit\"at G\"ottingen, G\"ottingen, Germany}
\affil[43]{Kavli Institute for Cosmology, University of Cambridge, Cambridge, United Kingdom}
\affil[44]{Cavendish Laboratory, University Cambridge, Cambridge, United Kingdom}
\affil[45]{Department of Physics, Californina State University - East Bay, Hayward, California, USA}
\affil[46]{Institut fuer theoretische Physik, Universitaet Heidelberg, Heidelberg, Germany}
\affil[47]{Department of Physics, University of Illinois at Urbana-Champaign, Urbana, IL, USA}
\affil[48]{Illinois Institute of Technology, Chicago, IL, USA}
\affil[49]{Physikalisch-Technische Bundesanstalt, Braunschweig, Germany}
\affil[50]{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA, USA}
\affil[51]{Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA, USA}
\affil[52]{Max-Planck-Institut f\"ur Physik, Munich, Germany}
\affil[53]{JILA, National Institute of Standards and Technology and University of Colorado, Boulder, CO, USA}
\affil[54]{National Institute of Standards and Technology, Boulder, CO, USA}
\affil[55]{Department of Physics, University of Colorado, Boulder, CO, USA}
\affil[56]{Deutsches Elektronen-Synchrotron DESY, Hamburg, Germany}
\affil[57]{Max-Planck-Institut f\"ur Kernphysik, Heidelberg, Germany}
\affil[58]{Theoretical Particle Physics and Cosmology, King's College London, London, United Kingdom}
\affil[59]{ARC Centre of Excellence for Dark Matter Particle Physics, Deptartment of Physics, The University of Western Australia, Crawley, WA, Australia}
\affil[60]{ARC Centre of Excellence for Dark Matter Particle Physics, Swinburne University of Technology, John St, Hawthorn VIC 3122, Australia}
\affil[61]{Nordita, KTH Royal Institute of Technology and Stockholm University, Stockholm, Sweden}
\affil[62]{University of Florida, Gainesville, FL, USA}
\affil[63]{The National Aeronautics and Space Administration (NASA), Washington, D.C., USA}
\affil[64]{School of Physics, The University of Sydney, Camperdown, NSW, Australia}
\affil[65]{Yale Center for Astronomy and Astrophysics, Department of Physics, Yale University, New Haven, Connecticut, USA}
\affil[66]{Dunlap Institute for Astronomy \& Astrophysics, University of Toronto, Toronto, ON, Canada}
\affil[67]{Department of Physics and Astronomy, University of Delaware, Newark, DE, USA}
\affil[68]{CAS Key Laboratory of Theoretical Physics, Institute of Thereotical Physics, Chinese Academy of Science, Beijing, P.R.China}
\affil[69]{Department of Electrical and Computer Engineering, University of Delaware, Newark, DE, USA}
\affil[70]{Department of  Physics and Astronomy, University of Oklahoma, Norman, OK, USA}
\affil[71]{Indiana University Center for Spacetime Symmetries, Bloomington, IN, USA}
\affil[72]{Johns Hopkins University, Baltimore, MD, USA}
\affil[73]{Boston Universitry, Boston, MA, USA}
\affil[74]{University of California, Irvine, Irvine, CA, USA}
\affil[75]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), UTIAS, The University of Tokyo, Kashiwa, Japan}
\affil[76]{Tsung-Dao Lee Institute, Shanghai, P.R. China}
\affil[77]{School of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai, P.R. China}
\affil[78]{University of California, Los Angeles, Los Angeles, CA, USA}
\affil[79]{Center for Cosmology and Particle Physics, Department of Physics, New York University, New York, NY, USA}
\affil[80]{Santa Clara University, Santa Clara, CA, USA}
\affil[81]{PRISMA$^+$ Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, Mainz, Germany}
\affil[82]{School of Physics and Astronomy, Tel-Aviv University, Tel-Aviv 69978, Israel}


